On the Distribution of "Simple Stupid Bugs" in Unit Test Files: An Exploratory Study

A key aspect of ensuring the quality of a software system is the practice of unit testing. Through unit tests, developers verify the correctness of production source code, thereby verifying the system's intended behavior under test. However, unit test code is subject to issues, ranging from bugs in the code to poor test case design (i.e., test smells). In this study, we compare and contrast the occurrences of a type of single-statement-bug-fix known as "simple stupid bugs" (SStuBs) in test and non-test (i.e., production) files in popular open-source Java Maven projects. Our results show that SStuBs occur more frequently in non-test files than in test files, with most fix-related code associated with assertion statements in test files. Further, most test files exhibiting SStuBs also exhibit test smells. We envision our findings enabling tool vendors to better support developers in improving the maintenance of test suites.

==> temp.tex <==
\item clone the 100 maven prjs. use this for test file rqs
    \item Get issue tracker details
    \item LDA for each category
    \item LDA on bug fix commit - compare ssbug vs other
    \item Test vs. Production
    \item Who creates vs. Who fixes
    \item does refactoring fix bugs? refminer on bugfix commit
    \item smells and bugs (before/after smell count)
    \item Revert fix 
    \item same issue reoccurs (same person fixes it)
    \item run tools - "understand"; code readability
